Correction of Errors in Preference Ratings from Automated Metrics for Text Generation

A major challenge in the field of Text Generation is evaluation: Human evaluations are cost-intensive, and automated metrics often display considerable disagreement with human judgments. In this paper, we propose a statistical model of Text Generation evaluation that accounts for the error-proneness of automated metrics when used to generate preference rankings between system outputs. We show that existing automated metrics are generally over-confident in assigning significant differences between systems in this setting. However, our model enables an efficient combination of human and automated ratings to remedy the error-proneness of the automated metrics. We show that using this combination, we only require about 50% of the human annotations typically used in evaluations to arrive at robust and statistically significant results while yielding the same evaluation outcome as the pure human evaluation in 95% of cases. We showcase the benefits of approach for three text generation tasks: dialogue systems, machine translation, and text summarization.

==> tables/naive_results_small.tex <==
\begin{tabular}{ l | c c c c | c}
Metric & Corr. & Inv. & Mis. & Red. & KLD \\\hline 
\multicolumn{ 6 }{c}{Chatbot Domain} \\ \hline
deb      & 0.60 & 0.00 & 0.07 & 0.33 & 0.39\\
grade    & 0.53 & 0.07 & 0.20 & 0.20 & 0.53\\
holistic & 0.27 & 0.20 & 0.13 & 0.40 & 0.57\\
maude    & 0.40 & 0.13 & 0.13 & 0.33 & 0.42\\
usl      & 0.53 & 0.07 & 0.00 & 0.40 & 0.40\\ \hline \hline
\multicolumn{ 6 }{c}{Summeval Relevance Domain} \\ \hline
BertScore & 0.63 & 0.13 & 0.03 & 0.22 & 0.28\\
BLANC     & 0.49 & 0.23 & 0.03 & 0.25 & 0.28\\
CIDEr     & 0.43 & 0.28 & 0.04 & 0.25 & 0.38\\
ROUGE-L   & 0.51 & 0.23 & 0.03 & 0.23 & 0.28\\
S3        & 0.60 & 0.15 & 0.03 & 0.23 & 0.29\\
SummaQA   & 0.59 & 0.11 & 0.08 & 0.22 & 0.26\\
SUPERT    & 0.49 & 0.20 & 0.07 & 0.24 & 0.37\\ 
Ideal-$\mathcal{M}$ & 0.75 & 0.00 & 0.00 & 0.25 & 0.02 \\ \hline \hline
\multicolumn{ 6 }{c}{WMT21 Domain} \\ \hline
BleuRT & 0.47 & 0.02 & 0.13 & 0.38 & 0.46\\
C-SPEC & 0.78 & 0.00 & 0.07 & 0.15 & 0.53\\
COMET  & 0.40 & 0.09 & 0.13 & 0.38 & 0.65\\
BLEU   & 0.44 & 0.16 & 0.07 & 0.33 & 0.43\\ \hline
\end{tabular}


==> texsubfiles/OLDTEXT.tex <==
%\subsection{Oracle Case}
%We start the discussion with the oracle case, that is, given an error-free metric, how can we measure whether $\pi_1$ is better than $\pi_2$? 
%More precisely, how many comparisons are needed in order to measure whether the difference between $\pi_1$ and $\pi_2$ is significant?
%Let $n_{g} = \sum_{j=1}^{n} \mathbb{I}^{>}[r_j^o]$ denote the number of times $o_j^1$ was rated as being better than $o_j^2$. We analogously define  $n_{l} = \sum_{j=1}^{n} \mathbb{I}^{<}[r_j^o]$ the number of times $o_j^1$ was rated as being worse than $o_j^2$, and $n_{e} = \sum_{j=1}^{n} \mathbb{I}^{=}[r_j^o]$ the number of draws. For our framework, we interpret $n_{g,e,l}$ as observations, which are sampled from a Trinomial distribution with outcome probabilities $p_g, p_e$, and $p_l$ respectively. Thus, we can treat the outcomes as random variables, and describe the probability of a specific outcome as: 
%%\begin{equation*}
%\begin{aligned}
%     &P(N_g = n_g, N_e = n_e, N_l = n_l) \\
%     &= \frac{n!}{n_g!n_e!n_l!} p_g^{n_g}p_e^{n_e}p_l^{n_l}
%\end{aligned}
%\end{equation*}
%This allows us to derive a significance test for a Trinomial distribution based on paired data, which was proposed by~\citet{bian2011trinomial}. This leads to the following Theorem (the full derivations and proofs are found in Appendix~\ref{sec:derivations}). \begin{theorem}[Significant Difference]
%For given counts of $n_{g}$ and $n_{l}$, the difference between two text generation systems $\pi_1$ and $\pi_2$ is significant at the level $\gamma$ if $|\frac{n_{>} - n_{<}}{\sqrt{n_{>} + n_{<}}}| > \Phi^{-1}(1 - \frac{\gamma}{2})$, where $\Phi^{-1}$ is the inverse cumulative distribution function of the standard normal distribution. 
%\end{theorem}

%The above result is based on the frequentest view. Here, we introduce the Bayesian view, which will be useful in the subsequent discussion. For this we treat the probability distribution as a random variable, thus, the conjugate prior of the Trinomial distribution is the Dirichlet distribution $\bm{p} = (p_g, p_e, p_l) \sim Dirichlet(\alpha)$. This allows us to define the posterior distribution $p(\bm{p} | N_g = n_g, N_e = n_e, N_l = n_l) \propto Dirichlet(n_g + 1, n_e + 1, n_l + 1)$, which is based on the observed data $n_k$. Note that the expected value of the Dirichlet posterior for $p_k = \frac{n_k}{\sum_{j \in \{g,e,l\}}n_j}$, thus, equivalent to the maximum likelihood estimate above. Using Markov Chain Monte Carlo (MCMC) sampling from the posterior, we can determine whether $p_g > p_l$, which yields the same interpretation as the significance test above (see Appendix~\ref{sec:mcmc_samp} for the details). 

%\subsection{Error-Prone Case}
%We now discuss how to apply comparative metrics that make mistakes in their judgments. We cover two subcases: one where the mixture matrix $\bm{\mu}$ is known, and the other where $\bm{\mu}$ must be estimated from data. The first case introduces one level of uncertainty, i.e., we cannot be sure which samples are rated correctly by the metric. The second case introduces a second level of uncertainty, i.e., we cannot be sure about the values of $\bm{\mu}$. The Bayesian framework allows us to integrate all these levels of uncertainties. 

%For the rest of the discussion let $r_j^m = M^{ic}_c(i_j, \pi_1(i_j), \pi_2(i_j))$ denote the rating given by an error-prone metric. Analogous to before, we define $m_{g} = \sum_{j=1}^{n} \mathbb{I}^{>}[r_j^m]$ the number of times the error-prone metric rates the output of system $\pi_1$ to be better than those from $\pi_2$. The counts for equality and being worse are denoted by $m_e$ and $m_l$ respectively. Since $M^{ic}$ is an error-prone metric, the counts $m_{g,e,l}$ are not the true counts $n_{g,e,l}$ yielded by an oracle or error-free metric. Thus the goal is to use $\bm{\mu}$ to estimate the true counts $n_{g,e,l}$ from the observed ones $m_{g,e,l}$. We note that the true probabilities $\bm{p} = (p_g, p_e, p_l)$ are transformed by the mixture matrix to the error-prone ones by $\hat{\bm{p}} = (\hat{p_g}, \hat{p_e}, \hat{p_l}) = \bm{\mu} \bm{p}$.

%\subsection{Known $\bm{\mu}$}
%Here, we assume that the true mixture matrix $\bm{\mu}$ is known. Thus, we can estimate the true probability distribution $\bm{p} = \bm{\mu}^{-1}\hat{\bm{p}}$, where $\hat{\bm{p}} = (\frac{m_g}{n}, \frac{m_e}{n}, \frac{m_l}{n})$ is the maximum likelihood estimate. In Bayesian terms, we combine the prior belief of the true value of $\bm{p}$ with the likelihood of the observed $m_{g,e,l}$ values.
%\begin{equation*}\label{eq:fixed_mu}
%    \begin{aligned}
%        &p_g, p_e, p_l \sim Dirichlet(\alpha) \\
%        &m_>, m_=, m_< | \bm{p} \sim Trinomial(n, \bm{\mu}\bm{p}) \\
%        &p(\bm{p} | m_>, m_=, m_<)\\ 
%        &\propto P(M_> = m_>, M_= = m_=, M_< = m_< | \bm{p})p(\bm{p}) 
%    \end{aligned}
%\end{equation*}

%The hyperparameters $\alpha$ are either set to $1$ when we do not have any prior information, or we can incorporate the belief derived from comparison oracle ratings as in the previous section. This allows to combine error-free measurements with error-prone measurements.  Note that we are not aware of any closed form solution for the above formula, thus, we apply Markov Chain Monte Carlo (MCMC) sampling to sample the posterior distribution $p(\bm{p} | m_>, m_=, m_<)$ and determine whether $p_g > p_l$, i.e., the probability that system $\pi_1$ is better than system $\pi_2$.

%\subsection{Estimated $\bm{\mu}$}
%In a real-world scenario the values of $\bm{\mu}$ must be estimated from data. This is achieved by comparing the error-prone metric outputs to a set of error-free metric outputs, that is:
%\begin{equation*}
%\small
%    \begin{aligned}
%        &n_{mo} = \sum_{i = 1}^{n} \mathbb{I}[r_j^m = m] \land \mathbb{I}[r_j^o = o] ,\forall m, o \in \{>, =, <\} \\
%        &\hat{\mu}_{mo} = \frac{n_{mo}}{\sum_{k \in \{>, =, <\}} n_{mk}}
%    \end{aligned}
%\end{equation*}

%In Bayesian terms, we treat each row in the mixture matrix as a probability distribution, which can be modeled as a Dirichlet distribution.
%\begin{equation*}\label{eq:mu:diriclet}
%\small
%    \begin{aligned}
%        &\bm{\mu_{\cdot>}} = (\mu_{>>}, \mu_{=>}, \mu{<>})^\top \sim Dirichlet(\alpha_>) \\
%        &\bm{\mu_{\cdot=}} = (\mu_{>=}, \mu_{==}, \mu{<=})^\top  \sim Dirichlet(\alpha_=) \\
%        &\bm{\mu_{\cdot<}} = (\mu_{><}, \mu_{=<}, \mu_{<<})^\top \sim Dirichlet(\alpha_<) \\
%        &\bm{\mu} = (\bm{\mu_{\cdot>}}, \bm{\mu_{\cdot=}}, \bm{\mu_{\cdot<}}) \\
%    \end{aligned}
%\end{equation*}
%where $\alpha_>$ denotes all the counts for this row, i.e., $n_{>>} + 1, n_{=>} + 1, n_{<>} + 1$. Thus, we treat $\bm{\mu}$ as a vector of Dirichlet distributions. From these, we estimate the %probability distribution $\bm{p}$ as follows: 
%\begin{equation*}\label{eq:comp_full_bayes}
%\small
%    \begin{aligned}
%        &\bm{p} = (p_>, p_=, p_<)^\top  \sim Dirichlet(\alpha) \\
%        & m_>, m_=, m_< | \bm{p}, \bm{\mu} \sim Trinomial(n, \bm{\mu}\bm{p}) \\
%        & p(\bm{p}, \bm{\mu} | m_>, m_=, m_<) \propto
%        P(m_>, m_=, m_< | \bm{p}, \bm{\mu})p(\bm{p})p(\bm{\mu}) \\
%    \end{aligned}
%\end{equation*}

%Since we are not aware of any closed form solutions to the above formula, we apply Markov Chain Monte Carlo (MCMC) sampling to sample both $\bm{p}$ and $\bm{\mu}$ from the posterior distribution.
